MeerCRAB: MeerLICHT Classification of Real and Bogus Transients using Deep Learning

Astronomers require efficient automated detection and classification pipelines when conducting large-scale surveys of the (optical) sky for variable and transient sources. Such pipelines are fundamentally important, as they permit rapid follow-up and analysis of those detections most likely to be of scientific value. We therefore present a deep learning pipeline based on the convolutional neural network architecture called $\texttt{MeerCRAB}$. It is designed to filter out the so called 'bogus' detections from true astrophysical sources in the transient detection pipeline of the MeerLICHT telescope. Optical candidates are described using a variety of 2D images and numerical features extracted from those images. The relationship between the input images and the target classes is unclear, since the ground truth is poorly defined and often the subject of debate. This makes it difficult to determine which source of information should be used to train a classification algorithm. We therefore used two methods for labelling our data (i) thresholding and (ii) latent class model approaches. We deployed variants of $\texttt{MeerCRAB}$ that employed different network architectures trained using different combinations of input images and training set choices, based on classification labels provided by volunteers. The deepest network worked best with an accuracy of 99.5$\%$ and Matthews correlation coefficient (MCC) value of 0.989. The best model was integrated to the MeerLICHT transient vetting pipeline, enabling the accurate and efficient classification of detected transients that allows researchers to select the most promising candidates for their research goals.

==> contents/3-ML_introduction.tex <==
% \section{Machine Learning Approach}\label{sec:ML_Intro}

% Machine Learning (ML) can be broadly categorized as \textit{supervised} or \textit{unsupervised}. ML has led to a paradigm shift in astronomy for more than two decades. Its application can be observed in various studies, namely, pulsar sifting using  ML \citep{2020arXiv200714843L}, a deep-learning classifier for Fast Radio Bursts (\texttt{FETCH}, \citealt{10.1093/mnras/staa1856}) and point source detection (\texttt{DEEPSOURCE}, \citealt{2019MNRAS.484.2793V}) to name a few. Concomitantly, Deep Learning (DL, \citealt{PMID:17921042}) and Convolutional Neural Networks (CNNs, \citealt{Lecun99objectrecognition}) have solved many complex image and speech recognition problems thereby revolutionising how ML is practically applied (\citealt{2014arXiv1406.2661G,2019MNRAS.485.5831L}). 

% In this paper we treat the identification of real and bogus transients as a supervised learning problem. Here for each input $\mathbf{x}$ there is an associated label/target value $\mathbf{y}$ describing its true class. The aim of supervised learning is to predict the label for $\mathbf{x}$ when $\mathbf{y}$ is unknown, usually by estimating $\mathsf{P}\left(y|x\right)$. 

%Next we introduce some deep learning terminology before describing the various layers used to construct the MeerCRAB model.



%\subsection{Deep Neural Network}
%The \texttt{MeerCRAB} model is composed of various layers, namely Convolutional Neural Network (CNN) plus pooling, dense and activation layers among others. A CNN is a type of Artificial Neural Network (ANN). It is a feed-forward neural network, deep learning models. The aim of an ANN is to approximate some function $f^{*}$. For instance, for a classification scenario $\mathbf{y} = f^{*}\left(\mathbf{x}\right)$ maps an input $\mathbf{x} \in \mathbb{R}^{n}$ to an output $\mathbf{y} \in \mathbb{R}^{m}$, which can also be written as

% \begin{equation}
%     \mathbf{y} = \alpha\left(\mathbf{Wx}+\mathbf{b}\right),
% 	\label{eq:MLPs}
% \end{equation}

%  \noindent where the matrix parameters $\mathbf{W} \in \mathbb{R}^{m \times n}$ are known as the \textit{weights}, a vector of small positive bias values $\mathbf{b}\in \mathbb{R}^{m}$ is called the \textit{biases} (can take values such as 0 or 0.1), and $\alpha$ is a non-linear activation function (see \S\ref{subsec:ReLU}). Therefore, an ANN is simply a mapping of $y=f\left(\mathbf{x};\mathbf{W},\mathbf{b}\right)$ and the algorithm learns the value of the parameters $\mathbf{W}$ and $\mathbf{b}$ that construct the best function approximation. In addition, ANNs consist of many different types of layers, which are detailed below.  

%  \subsubsection{Activation function: Rectified Linear Units (ReLU)}\label{subsec:ReLU}
% The activation function that is used after each CNN layer in \texttt{MeerCRAB} is the Rectified Linear Unit (ReLU). Most  activation functions can be viewed as taking an element-wise non-linear function $\alpha$ and apply it on top of an affine transformation $\mathbf{y} = \left(\mathbf{Wx}+\mathbf{b}\right)$. There are various other non-linear activation functions that are commonly used, for instance, \textit{sigmoid}, \textit{tanh}, \textit{ReLU} functions among others. The ReLU function can be defined as,

% \begin{equation}
%     \textrm{ReLU}\left(x\right) = \textrm{max}\big\{0,x\big\}.
% 	\label{eq:ReLU}
% \end{equation}

% \subsubsection{Softmax function}
% For the Real-Bogus classification scenario, the aim is to represent the output of our model by a probability distribution over a discrete variable. For the case of a classifier, the probability distribution is represented over $\mathbf{n}$ different classes and for the \texttt{MeerCRAB} model, since we are dealing with a binary classification problem we want to output a single number:

% \begin{equation}
% 	\hat{y} = \mathsf{P}\left(y=1|x\right),
% 	\label{eq:softmax_1}
% \end{equation}

% \noindent as this number has to lie between 0 and 1. The softmax function is used at the end of the network and it is given by:

% \begin{equation}
% 	\textrm{softmax}\left(x_{i}\right) = \frac{\textrm{exp}\left(x_{i}\right)}{\sum_{j=1}^{D}\textrm{exp}\left(x_{j}\right)},
% 	\label{eq:softmax}
% \end{equation}

% \noindent where $i\in \big\{1, \ldots ,D\big\}$ and \textit{D} is the number of neurons in the last \textit{dense} layer of the network. Formally, the softmax function is useful for multi-class-classification. For the case of binary classification, \textit{D} will be equal to 2 and the softmax function will assign a probability to each neuron. 


% \subsection{Convolutional Layers (CLs)}
% The \texttt{MeerCRAB} model is based mostly on CNN. The latter is a specialized type of neural network to process 1-D grid data for example, time-series, 2-D grid or 3-D grid of image pixels. CNN is a kind of linear operation and employs a mathematical operation to the input, called `convolution` which can be written as

% \begin{equation}
%     S = \alpha\left(\mathbf{x} * \mathbf{W} + \mathbf{b} \right),
% 	\label{eq:CLs}
% \end{equation}

% \noindent where $\mathbf{W}$ is the kernel or filter, $\mathbf{b}$ is the vector of biases for each filter, $\alpha$ is the activation function and the output $S$ is also known as the feature map.

% \subsubsection{Pooling layers}
% A typical CNN comprises of three stages. The first stage of the process performs several convolution operations that produces a sample of linear activations or feature maps as discussed above. At the second stage, each linear feature map is passed through a hidden units or a non-linear activation function, such as the \textit{ReLU} activation function described in \S\ref{subsec:ReLU} . The second stage is also known as the \textbf{detector stage}. Finally, the third stage deals with a \textbf{pooling} function that replaces the output of the network with the maximum output within a rectangular grid, also known as \textbf{Max Pooling}. The pooling function is an important step that enables the representation of the input \textit{invariant} to small translations. This helps to provide useful information about the presence of some features in the input rather than exactly where the features are located in the image.







% \subsection{Training neural network}
% After assembling the various layers of \texttt{MeerCRAB}, we then proceed with the training process. However, when training a ML algorithm, we need to specify an optimization function, a cost/loss function and a model structure. Therefore, during training we need to initialise all weights $\mathbf{W}$ to small random values and biases $\mathbf{b}$ to be initialised to 0 or small positive values. We adopt a supervised learning approach for training \texttt{MeerCRAB}. Hence we use labeled image data as input to the \texttt{MeerCRAB} model structure and then at the end of the process, we obtain classification probabilities. This stage is known as forward propagation. The difference between the true label and the classification probabilities is quantified by a cost function. An iterative gradient-based optimization algorithm is applied to train the DL models. The training process is mostly based on utilising the gradient to descend the cost function with respect to different weights. The gradient, together with a constant value, also known as the \textit{learning rate} is used to optimized the weights. This process is known as back-propagation.

% As with many ML models, to be able to apply gradient-based learning, we need to choose a cost function to minimize and also at the end how to represent the output of the model. Most models are trained based on maximum likelihood. This implies that the cost function is simply the negative log-likelihood. This is similar to the cross-entropy between the training data and the model distribution. The cross-entropy or cost function is written as

% \begin{equation}
%     \textrm{J}(\theta) = - \mathbb{E}_{x,y\sim\hat{\mathsf{P}}_{\textrm{data}}}\log\mathsf{P}_{\textrm{model}}\left(\mathbf{y}|\mathbf{x}\right),
% 	\label{eq:cross-entropy}
% \end{equation}

% \noindent where $\mathbb{E}_{x,y\sim\hat{\mathsf{P}}_{\textrm{data}}}$ is the expectation of \textit{x}, \textit{y} with respect to an empirical distribution $\hat{\mathsf{P}}_{\textrm{data}}$. The form of the cost function varies from model to model, which depends on the specific form of $\log\mathsf{P}_{\textrm{model}}$.

% The network is trained on the training data and is then evaluated on the validation data. The training process continues until we obtain the best performance on the validation set. At the end of the process, the trained model is saved and then can be used to perform prediction on the test data. It is important to emphasize that during training, both the validation and test sets have not been seen by the network.

% In addition, the training process is done in small batches of training data as both the forward and backward propagation are intensive computations. When the entire training set has been used once during forward and backward propagation, this is known as an \textit{epoch}. The training process is computationally expensive and is done through several epochs. Afterwards, training stops when the performance criterion is met. It is fundamental to note that the training process often undergoes underfit or overfit. To overcome those issues, we use regularisation, data augmentation and early stopping in the \texttt{MeerCRAB} pipeline, which are discussed further below.


% \subsubsection{Data Augmentation}
% The best strategy for better generalisation of a ML model is to train it with large amounts of data. In practice, in supervised learning approach the amount of labeled data is limited. One way to tackle this challenge is to create synthetic data and add it during the training process. For classification task, this means that the classifier takes as input a complicated and high-dimensional vector $\mathbf{x}$ and map it with a single target $\mathbf{y}$. This implies that the main task a classifier is facing is that it needs to be invariant to various transformation. We therefore can generate new input $\left(\mathbf{x},\mathbf{y}\right)$ easily by applying a transformation on $\mathbf{x}$ inputs in our training sample.

% Data augmentation technique has been an effective method for classification problem. Images being of high dimension and consist of various variations/noises, are therefore easily simulated. Operations like translating, scaling, rotating the training input images by a few pixels can often improve generalization, although CNNs (the convolution and pooling techniques) already have this feature of being translational invariant.

% \subsubsection{Early Stopping}
% The training of large models shows over-fitting characteristics when we observe that the negative log-likelihood of the training process or the training error decreases steadily with number of epochs (number of training iterations over the datasets), but the validation set error starts to increase again. This scenario implies that a model with the best validation set error can be obtained (thus a better test set error) if the parameter setting is returned at the point in time where the lowest validation set error has been captured. For every epoch when the validation set error improves, a copy of the model parameters is stored. Therefore, for some pre-specified number of epochs, the training process stops when no improvement of the parameters over the best recorded validation set error is recorded. This strategy is called \textbf{early stopping}.

% Example figure
% \begin{figure*}
% 	\centering
% 	\includegraphics[width=0.8\textwidth]{Figures/meervetting-web-interface.pdf}
%     \caption{MeerVETTING web-interface to vet MeerLICHT candidates as real and bogus. Volunteers are provided with three images (new, reference, difference) that are cut-outs of the science images.}
%     \label{fig:meervetting-web-interface}
% \end{figure*}




